RiskWorld: Risk-Aware World Modeling with Flow-Guided Occupancy Evolution for Selective Trajectory Planning in Automated Driving

Safe motion planning in automated driving requires anticipating evolving traffic risks and deciding when to revise the current planned trajectory. We introduce RiskWorld, a risk-aware world modeling framework for shared occupancy forecasting and selective trajectory replacement. Spatial risk fields and temporal actor context are fused with visual bird's-eye-view features. Flow-guided evolution transports occupancy and scene features, while signed residuals correct occupancy after transport. One forecast is generated per planning step and reused across candidates. Each candidate is compared with a current-state persistence reference, yielding a nonnegative collision-score correction. The trajectory selected by current-world evaluation serves as the planning anchor and is replaced only when additional predicted risk triggers intervention and an alternative satisfies component-wise constraints on predicted risk and trajectory error. Candidate geometries remain unchanged. We evaluate RiskWorld for open-loop planning on nuScenes using camera features, annotation-derived current and historical actor states, and dataset-provided map context. RiskWorld achieves the lowest collision rate at a long evaluation horizon of 3 s, and the second-best average L2 error among various state-of-the-art baselines, while running at 11.5 FPS on a single NVIDIA RTX 4090 with 90.81 M parameters. Within-setting ablations show that RiskWorld achieves lower collision rates than the current-state rescoring baseline, while forecast reuse enables additional candidates to be evaluated at low marginal computational cost.

==> tables/table1_main_comp_compute_xtra.tex <==
```latex
\begin{table*}[t]
\caption{Planning performance and computational efficiency on nuScenes under the VAD/ST-P3 protocol.}
\label{tab:model_comparison}
\centering
\small
\setlength{\tabcolsep}{2.55pt}
\renewcommand{\arraystretch}{1.12}

\begin{tabular}{@{}l|cc|rr|rrrr|rrrr@{}}
\toprule
Method
& Input
& Aux. Sup.
& Params.
& FPS$_{\text{4090}}$
& \multicolumn{4}{c|}{L2 (m) $\downarrow$}
& \multicolumn{4}{c}{CR (\%) $\downarrow$} \\
\cmidrule(lr){6-9}
\cmidrule(lr){10-13}

& & &
(M) $\downarrow$
& $\uparrow$
& 1s & 2s & 3s & Avg.
& 1s & 2s & 3s & Avg. \\
\midrule

ST-P3~\cite{hu2022stp3}
& Camera
& \shortstack{Map \& Box\\\& Depth}
& -- & 1.60
& 1.33 & 2.11 & 2.90 & 2.11
& 0.23 & 0.62 & 1.27 & 0.71 \\

UniAD~\cite{hu2023uniad}
& Camera
& \shortstack{Map \& Box \& Motion\\\& Track \& Occ.}
& 125.00 & 1.80
& 0.44 & 0.67 & 0.96 & 0.69
& 0.04 & \rankthird{0.08} & 0.23 & 0.12 \\

VAD~\cite{jiang2023vad}
& Camera
& \shortstack{Map \& Box\\\& Motion}
& 58.36 & 4.50
& 0.41 & 0.70 & 1.05 & 0.72
& 0.07 & 0.17 & 0.41 & 0.22 \\

GenAD~\cite{zheng2024genad}
& Camera
& \shortstack{Map \& Box\\\& Motion}
& -- & --
& 0.28 & 0.49 & 0.78 & 0.52
& 0.08 & 0.14 & 0.34 & 0.19 \\

SparseDrive-S~\cite{sunSparseDriveEndtoEndAutonomous2025}
& Camera
& \shortstack{Map \& Box\\\& Motion \& Track}
& 85.90 & 9.00
& 0.29 & 0.58 & 0.96 & 0.61
& \rankfirst{0.01} & \ranksecond{0.05}
& \rankthird{0.18} & \ranksecond{0.08} \\

MomAD~\cite{song2025momad}
& Camera
& \shortstack{Map \& Box\\\& Motion}
& 87.00$^\dagger$ & 7.80
& 0.31 & 0.57 & 0.91 & 0.60
& \rankfirst{0.01} & \ranksecond{0.05}
& 0.22 & \rankthird{0.09} \\

DiffusionDrive~\cite{liao2025diffusiondrive}
& Camera
& \shortstack{Map \& Box\\\& Motion \& Track}
& 92.04 & 8.20
& 0.27 & 0.54 & 0.90 & 0.57
& \rankthird{0.03} & \ranksecond{0.05}
& \ranksecond{0.16} & \ranksecond{0.08} \\

LAW~\cite{liEnhancingEndtoEndAutonomous2024}
& Camera
& None
& 38.33 & --
& 0.26 & 0.57 & 1.01 & 0.61
& 0.14 & 0.21 & 0.54 & 0.30 \\

Drive-OccWorld~\cite{yang2025driveoccworld}
& Camera
& Occ. \& Flow
& -- & --
& 0.25 & \rankthird{0.44}
& \rankthird{0.72} & \rankthird{0.47}
& \rankthird{0.03} & \rankthird{0.08}
& 0.22 & 0.11 \\

World4Drive~\cite{zheng2025world4drive}
& Camera
& None
& 70.18 & --
& \rankthird{0.23} & 0.47 & 0.81 & 0.50
& \ranksecond{0.02} & 0.12 & 0.33 & 0.16 \\

ResWorld~\cite{zhangResWorldTemporalResidual2026}
& Camera
& None
& 80.77
& 10.3$^\ddagger$
& \rankfirst{0.17} & \rankfirst{0.32}
& \rankfirst{0.55} & \rankfirst{0.35}
& \rankfirst{0.01} & \rankfirst{0.02}
& \ranksecond{0.16} & \rankfirst{0.07} \\

\midrule

OccWorld-O~\cite{zheng2024occworld}
& GT Occ.
& Occ.
& -- & --
& 0.32 & 0.61 & 0.98 & 0.64
& 0.06 & 0.21 & 0.47 & 0.24 \\

\midrule

\textbf{RiskWorld (ours)}
& \shortstack{Camera \& Map\\\& GT Tracks}
& \shortstack{Risk/Occ.\\\& Collision}
& 90.81
& \textbf{11.5}& \ranksecond{0.18} & \ranksecond{0.37}
& \ranksecond{0.65} & \ranksecond{0.40}
& 0.06 & \rankthird{0.08}
& \rankfirst{0.14} & \rankthird{0.09} \\

\bottomrule
\end{tabular}

\smallskip

\begin{minipage}{\textwidth}
\footnotesize
Input refers to inference inputs; Aux.\ Sup.\ excludes ego-trajectory
supervision and generic backbone pretraining.
GT Tracks denotes current and historical ground-truth actor states.
FPS denotes inference throughput on a single NVIDIA RTX 4090 under
the nuScenes open-loop planning setting. Published RTX 4090
measurements are used where available; ``--'' indicates that a
comparable measurement was not found.
ResWorld throughput ($^\ddagger$) was measured locally on an NVIDIA
RTX 4090 using the authors' original implementation.
Parameter counts denote the online inference model where available.
Values for VAD, DiffusionDrive, LAW, World4Drive, and ResWorld are
computed from their released implementations or configurations;
$^\dagger$ denotes a value reported by a subsequent comparison rather
than the original method.
World4Drive excludes models used only for offline depth and mask
generation.
Gray highlights the top three distinct values in each planning metric;
bold and underline indicate first and second, including ties.
Efficiency columns are not included in the planning-metric ranking.
Input and supervision settings differ across methods.
\end{minipage}

\end{table*}
```


==> tables/table2_compute.tex <==
\begin{table}[!t]
\caption{Computational efficiency comparison.
FPS values measured on different GPUs are not directly comparable.}
\label{tab:efficiency_comparison}
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}lrrrl@{}}
\toprule
Method
& Params. $\downarrow$
& FLOPs $\downarrow$
& FPS $\uparrow$
& GPU \\
& (M) & (G) & & \\
\midrule
UniAD
& 125.00 & 1709.00 & 1.80 & A100 \\
VAD-Base
& 58.36 & -- & 4.50 & RTX 4090 \\
SparseDrive-S
& 85.90 & 192.00 & 9.00 & RTX 4090 \\
DiffusionDrive
& 92.04 & -- & 8.20 & RTX 4090 \\
LAW
& 38.33 & -- & -- & -- \\
World4Drive
& 70.18 & -- & -- & -- \\
\midrule
RiskWorld (ours)
& 90.81 & 1887.51 & 6.59 & A40 \\
\bottomrule
\end{tabular}

\smallskip
\begin{minipage}{\columnwidth}
\footnotesize
Parameter counts for VAD-Base, DiffusionDrive, LAW,
and World4Drive are computed from their released
configurations: R50, R50, Swin-Tiny without auxiliary
perception tasks, and R50 with $D=256$, respectively.
World4Drive excludes the models used for offline
depth and mask generation.
Other baseline values are taken from
SparseDrive~\cite{sunSparseDriveEndtoEndAutonomous2025}
and DiffusionDrive~\cite{liao2025diffusiondrive}.
``--'' indicates an unavailable value.
\end{minipage}
\end{table}

==> tables/table5_nuscene.tex <==
\begin{table}[!t]
\caption{Offline candidate replay on NAVSIM v1.1.}
\label{tab:navsim_offline}
\centering
\footnotesize
\vspace{-1.5mm}

\setlength{\tabcolsep}{2.5pt}
\renewcommand{\arraystretch}{0.88}
\setlength{\aboverulesep}{0.5pt}
\setlength{\belowrulesep}{0.5pt}

\begin{tabular*}{\columnwidth}{
@{\extracolsep{\fill}}l|r|r@{}}
\toprule
Method
& PDMS $\uparrow$
& {\scriptsize New safety failures $\downarrow$} \\
\midrule
TransFuser (C0)
& 89.8 & 0 \\
RiskWorld w/o gate
& \textbf{90.6} & 155 \\
RiskWorld
& 90.1 & \textbf{0} \\
\bottomrule
\end{tabular*}

\vspace{0.5mm}
\begin{minipage}{\columnwidth}
\raggedright
\scriptsize
Results use the same 6,561 held-out samples and K12 candidate pool.
New safety failures are additional NC/TTC/DAC/LK failures relative to C0.
\end{minipage}
\par\vspace{-9pt}

\end{table}
